Co-advise: Cross Inductive Bias Distillation

Transformers recently are adapted from the community of natural language processing as a promising substitute of convolution-based neural networks for visual learning tasks. However, its supremacy degenerates given an insufficient amount of training data (e.g., ImageNet). To make it into practical utility, we propose a novel distillation-based method to train vision transformers. Unlike previous works, where merely heavy convolution-based teachers are provided, we introduce lightweight teachers with different architectural inductive biases (e.g., convolution and involution) to co-advise the student transformer. The key is that teachers with different inductive biases attain different knowledge despite that they are trained on the same dataset, and such different knowledge compounds and boosts the student's performance during distillation. Equipped with this cross inductive bias distillation method, our vision transformers (termed as CivT) outperform all previous transformers of the same architecture on ImageNet.

==> 1.intro.tex <==

\section{Introduction}
\begin{figure}[t]
    \centering
    \begin{tabular}{c}
        \includegraphics[width=0.95\textwidth,height=3.5cm]{figs/teaser01.pdf}\\
        \includegraphics[width=0.95\textwidth,height=3.5cm]{figs/teaser02.pdf}\\
        \includegraphics[width=0.95\textwidth,height=3.5cm]{figs/teaser03.pdf}\\
    \end{tabular}\vspace{-3mm}
    \caption{Class probabilities predicted by a CNN, an INN, a transformer without distillation, and a transformer distilling from both CNN and INN. CNN and INN provide come up with consistent (the first row) or complementary (the second and third rows) conclusions to correct transformer's prediction.}
  \label{fig:cnn_inn_transf_bef_aft_distill}
\end{figure}
With the advent of LeNet \cite{LeNet} around thirty years ago, convolution operator was introduced into the area of computer vision \cite{LeNet,LeCun_handwritten}. By enabling the convolutional neural network (CNN) to go deep in the past decade, we witnessed its supremacy in various tasks (e.g.\ image classification \cite{AlexNet}, object detection \cite{ResNet,fpn}, semantic segmentation \cite{seg_nyu_depth}). Consequently, deep CNNs become the critical building block and the \textit{de facto} choice for learning tasks in computer vision.  

Albeit the flourish of the convolution operator, it does possess certain limitations. The major one is that convolution operator processes in a spatial neighborhood, thereby making spatially-distant interactions difficult to be captured \cite{nonlocalnet,vt}. Motivated by this observation, vast research interests have been intrigued in replacing convolution layers with novel architectures \cite{nonlocalnet,involution,vit,dert,vt,deit}. Along this line of research, self-attention-based architectures (a.k.a.\ transformers \cite{attention_is_all_u_need}) form a notable mainstream \cite{vit,dert,vt} at present. For instance, ViT \cite{vit}, a pure transformer without convolutional layers, achieves state-of-the-art (SOTA) accuracy when trained on large datasets (e.g., JFT-300M).

Nevertheless, when only mid-sized datasets (e.g., ImageNet \cite{imagenet}) are available, ViT (or more generally, transformers) usually couldn't reveal better performances compared to its convolutional counterparts \cite{vit,deit}. The intrinsic reason is that transformers lack inductive biases inherent in CNNs (e.g., translation equivariance and locality) and thus do not generalize well given insufficient amounts of data \cite{vit}. In this context, knowledge distillation technique \cite{hinton2015distilling,furlanello2018born} is further applied by \cite{deit} to assist the training of transformers. Specifically, provided a pre-trained convolutional teacher model, the DeiT proposed in \cite{deit} is able to achieve competitive results as CNNs on ImageNet. However, such transformer distilled from a CNN is too biased towards convolution teachers and is placed restrictions on the inductive bias of the teacher. Besides, the heavy convolution teacher (RegNetY-16GF) in DeiT becomes the computational burden in the whole training process.

Recently, the emerging of involution-based neural networks (INNs) \cite{involution} equips us with a new weapon and yields overall three architectures (i.e., CNNs, transformers, INNs) available to solve learning tasks in vision. In this paper, we propose a cross inductive bias distillation method to train a vision transformer. We leverage both an INN and a CNN as teacher models, for which we believe that their inverse inherent inductive biases (spatial-agnostic and channel-specific in convolution, spatial-specific and channel-agnostic in involution) could drive them to harvest different knowledge even training on the same dataset (see Figure \ref{fig:cnn_inn_transf_bef_aft_distill}). Such different inductive biases in the teacher could provide different aspects to describe same data, perceives the data differently and makes different assumptions of the data. In contrast, teachers with the same inductive biases but different performance (e.g., ResNet-18 and ResNet-50) have little difference in data description. Based on these advantages, there are only two super lightweight cross inductive bias teachers to be required in our methods. In the following step, these knowledge could compensate each other and ultimately prompt the accuracy of the student transformer. The main contribution of our paper is summarized as follows:
\begin{itemize}
    \item Our proposed cross inductive bias vision transformer (CivT) outperforms all previous distillation-based vision transformers on ImageNet and only needs to equip with super lightweight teachers whose total parameters are less than one-fifth of those of DeiT-Ti and a half of those of DeiT-S respectively.
    \item We observe that compared to the performance of a teacher model, its intrinsic inductive biases might even impact more on the student model.
    \item CNNs and INNs are inclined to learn texture and structure relationship respectively, while a vision transformer, a more general architecture with fewer inductive biases, could inherit useful knowledge from both.
    \item When several teacher models with different inductive biases are provided, it is beneficial to choose a student model possessing few inductive biases.
\end{itemize}

The remainder of this paper is organized as follows. In Section \ref{section:related_work}, we briefly review some preliminary concepts. Next, we propose our cross inductive bias distillation method in Section \ref{section:proposed_method}. The efficacy of our method is thoroughly verified in Section \ref{section:experiment}. Finally, we conclude in Section \ref{section:conclusion}.
 
 






